Weak mixing in rational billiards

We completely characterize rational polygons whose billiard flow is weakly mixing in almost every direction as those which are not almost integrable, in the terminology of Gutkin, modulo some low complexity exceptions. This proves a longstanding conjecture of Gutkin. This result is derived from a complete characterization of translation surfaces that are weakly mixing in almost every direction: they are those that do not admit an affine factor map to the circle.

==> bibliography.tex <==
@ARTICLE{CF,
       author = {{Chaika}, Jon and {Forni}, Giovanni},
        title = "{Weakly Mixing Polygonal Billiards}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Dynamical Systems, Mathematics - Geometric Topology, 37A25, 37E35, 30F60, 32G15},
         year = 2020,
        month = mar,
          eid = {arXiv:2003.00890},
        pages = {arXiv:2003.00890},
          doi = {10.48550/arXiv.2003.00890},
archivePrefix = {arXiv},
       eprint = {2003.00890},
 primaryClass = {math.DS},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv200300890C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{CD,
       author = {{Chaika}, Jon and {Davis}, Diana},
        title ="{The typical measure preserving transformation is not an interval exchange transformation}",
      journal = {prerint, arXiv:1812.10425v1},
     keywords ={} ,
         year = 2018,
       month = { },
     eid = { },
        pages = {1--9},
          doi = { },
archivePrefix = {},
       eprint = { },
 primaryClass = {math.DS},
adsurl = { },
      adsnote = {https://arxiv.org/abs/1812.10425}
}

@article {FOD,
    AUTHOR = {Wright, Alex},
     TITLE = {The field of definition of affine invariant submanifolds of
              the moduli space of abelian differentials},
   JOURNAL = {Geom. Topol.},
  FJOURNAL = {Geometry \& Topology},
    VOLUME = {18},
      YEAR = {2014},
    NUMBER = {3},
     PAGES = {1323--1341},
      ISSN = {1465-3060,1364-0380},
   MRCLASS = {32G15 (30F60 37D40)},
  MRNUMBER = {3254934},
MRREVIEWER = {Jayadev\ S.\ Athreya},
       DOI = {10.2140/gt.2014.18.1323},
       URL = {https://doi.org/10.2140/gt.2014.18.1323},
}

@article {EMM,
    AUTHOR = {Eskin, Alex and Mirzakhani, Maryam and Mohammadi, Amir},
     TITLE = {Isolation, equidistribution, and orbit closures for the {${\rm
              SL}(2,\mathbb R)$} action on moduli space},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {182},
      YEAR = {2015},
    NUMBER = {2},
     PAGES = {673--721},
      ISSN = {0003-486X,1939-8980},
   MRCLASS = {58D27 (22F10 32G15 37C85 37D40 60B15)},
  MRNUMBER = {3418528},
MRREVIEWER = {Boris\ Hasselblatt},
       DOI = {10.4007/annals.2015.182.2.7},
       URL = {https://doi.org/10.4007/annals.2015.182.2.7},
}

@article {EM,
    AUTHOR = {Eskin, Alex and Mirzakhani, Maryam},
     TITLE = {Invariant and stationary measures for the {${\rm SL}(2,\mathbb R)$} action on moduli space},
   JOURNAL = {Publ. Math. Inst. Hautes \'{E}tudes Sci.},
  FJOURNAL = {Publications Math\'{e}matiques. Institut de Hautes \'{E}tudes
              Scientifiques},
    VOLUME = {127},
      YEAR = {2018},
     PAGES = {95--324},
      ISSN = {0073-8301,1618-1913},
   MRCLASS = {37D40 (22E50 37C85)},
  MRNUMBER = {3814652},
MRREVIEWER = {Thomas\ Ward},
       DOI = {10.1007/s10240-018-0099-2},
       URL = {https://doi.org/10.1007/s10240-018-0099-2},
}

@article {mono,
    AUTHOR = {Filip, Simion},
     TITLE = {Zero {L}yapunov exponents and monodromy of the
              {K}ontsevich-{Z}orich cocycle},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {166},
      YEAR = {2017},
    NUMBER = {4},
     PAGES = {657--706},
      ISSN = {0012-7094,1547-7398},
   MRCLASS = {37D25 (14D07 32G15 37D40)},
  MRNUMBER = {3619303},
MRREVIEWER = {Jayadev\ S.\ Athreya},
       DOI = {10.1215/00127094-3715806},
       URL = {https://doi.org/10.1215/00127094-3715806},
}

@article{Gu84, 
title={Billiards on almost integrable polyhedral surfaces}, 
volume={4}, 
DOI={10.1017/S0143385700002650}, 
number={4}, 
journal={Ergodic Theory and Dynamical Systems}, 
author={Gutkin, E.}, 
year={1984}, 
pages={569–584}} 

@article{Gu86,
title = {Billiards in polygons},
journal = {Physica D: Nonlinear Phenomena},
volume = {19},
number = {3},
pages = {311-333},
year = {1986},
issn = {0167-2789},
doi = {https://doi.org/10.1016/0167-2789(86)90062-X},
url ={https://www.sciencedirect.com/science/article/pii/016727898690062X},
author = {Eugene Gutkin},
abstract = {We report on the state of the art for billiards in polygons.}
}
@InProceedings{GK88,
author="Gutkin, E.
and Katok, A.",
editor="Gomez-Mont, Xavier
and Seade, Jos{\'e} A.
and Verjovski, Alberto",
title="Weakly mixing billiards",
booktitle="Holomorphic Dynamics",
year="1988",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="163--176",
isbn="978-3-540-45957-6"
}
@article {AvFo,
    AUTHOR = {Avila, Artur and Forni, Giovanni},
     TITLE = {Weak mixing for interval exchange transformations and
              translation flows},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {165},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {637--664},
      ISSN = {0003-486X,1939-8980},
   MRCLASS = {37A25 (28D05 37D40 37E35)},
  MRNUMBER = {2299743},
MRREVIEWER = {Gabriela\ Schmith\"usen},
       DOI = {10.4007/annals.2007.165.637},
       URL = {https://doi.org/10.4007/annals.2007.165.637},
}

@article {NoRu,
    AUTHOR = {Nogueira, A. and Rudolph, D.},
     TITLE = {Topological weak-mixing of interval exchange maps},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {17},
      YEAR = {1997},
    NUMBER = {5},
     PAGES = {1183--1209},
      ISSN = {0143-3857,1469-4417},
   MRCLASS = {58F19 (54H20 58F11)},
  MRNUMBER = {1477038},
MRREVIEWER = {Pierre\ Arnoux},
       DOI = {10.1017/S0143385797086276},
       URL = {https://doi.org/10.1017/S0143385797086276},
}

@article {AvDe,
    AUTHOR = {Avila, Artur and Delecroix, Vincent},
     TITLE = {Weak mixing directions in non-arithmetic {V}eech surfaces},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {29},
      YEAR = {2016},
    NUMBER = {4},
     PAGES = {1167--1208},
      ISSN = {0894-0347,1088-6834},
   MRCLASS = {37A05 (37E35)},
  MRNUMBER = {3522612},
MRREVIEWER = {Jayadev\ S.\ Athreya},
       DOI = {10.1090/jams/856},
       URL = {https://doi.org/10.1090/jams/856},
}
@article {AvLe,
    AUTHOR = {Avila, Artur and Leguil, Martin},
     TITLE = {Weak mixing properties of interval exchange transformations \&
              translation flows},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'et\'e{} Math\'ematique de France},
    VOLUME = {146},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {391--426},
      ISSN = {0037-9484,2102-622X},
   MRCLASS = {37E35 (37A25 37E05)},
  MRNUMBER = {3933880},
MRREVIEWER = {Lanyu\ Wang},
       DOI = {10.24033/bsmf.2761},
       URL = {https://doi.org/10.24033/bsmf.2761},
}
@article {Vmetric,
    AUTHOR = {Veech, William A.},
     TITLE = {The metric theory of interval exchange transformations. {I}.
              {G}eneric spectral properties},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {106},
      YEAR = {1984},
    NUMBER = {6},
     PAGES = {1331--1359},
      ISSN = {0002-9327,1080-6377},
   MRCLASS = {28D05 (28D20 58F11)},
  MRNUMBER = {765582},
MRREVIEWER = {Andr\'es\ del\ Junco},
       DOI = {10.2307/2374396},
       URL = {https://doi.org/10.2307/2374396},
}

@article{MW18,
author = {Maryam Mirzakhani and Alex Wright},
title = {{Full-rank affine invariant submanifolds}},
volume = {167},
journal = {Duke Mathematical Journal},
number = {1},
publisher = {Duke University Press},
pages = {1 -- 40},
keywords = {Abelian differential, affine invariant submanifold, Hodge bundle, rational billiards, Riemann surface, Teichm√ºller dynamics, translation surface},
year = {2018},
doi = {10.1215/00127094-2017-0036},
URL = {https://doi.org/10.1215/00127094-2017-0036}
}

@book {Kec,
    AUTHOR = {Kechris, Alexander S.},
     TITLE = {Classical descriptive set theory},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {156},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1995},
     PAGES = {xviii+402},
      ISBN = {0-387-94374-9},
   MRCLASS = {03E15 (03-01 03-02 04A15 28A05 54H05 90D44)},
  MRNUMBER = {1321597},
MRREVIEWER = {Jakub\ Jasi\'nski},
       DOI = {10.1007/978-1-4612-4190-4},
       URL = {https://doi.org/10.1007/978-1-4612-4190-4},
}

@article {BoNo,
    AUTHOR = {Boshernitzan, Michael and Nogueira, Arnaldo},
     TITLE = {Generalized eigenfunctions of interval exchange maps},
   JOURNAL = {Ergodic Theory Dynam. Systems},
  FJOURNAL = {Ergodic Theory and Dynamical Systems},
    VOLUME = {24},
      YEAR = {2004},
    NUMBER = {3},
     PAGES = {697--705},
      ISSN = {0143-3857,1469-4417},
   MRCLASS = {37A25 (47A35)},
  MRNUMBER = {2060994},
MRREVIEWER = {Habib\ Marzougui},
       DOI = {10.1017/S0143385704000021},
       URL = {https://doi.org/10.1017/S0143385704000021},
}

@article {KMS,
    AUTHOR = {Kerckhoff, Steven and Masur, Howard and Smillie, John},
     TITLE = {Ergodicity of billiard flows and quadratic differentials},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {124},
      YEAR = {1986},
    NUMBER = {2},
     PAGES = {293--311},
      ISSN = {0003-486X,1939-8980},
   MRCLASS = {58F17 (30F30 58F11)},
  MRNUMBER = {855297},
MRREVIEWER = {Eugene\ Gutkin},
       DOI = {10.2307/1971280},
       URL = {https://doi.org/10.2307/1971280},
}

@article{Ma82,
  author		= "Masur, H.",
  title			= "Interval {E}xchange {T}ransformations and {M}easured {F}oliations",
  journal		= "Ann. of Math.",
  volume		= "115",
  number           =  "1",
  pages			= "169--200",
  year			= "1982"
}

@article{Ma85,
  author		= "Masur, H.",
  title			= "Ergodic {A}ctions of the {M}apping {C}lass {G}roup",
  journal		= "Proc.  Amer. Math. Soc.",
  volume		= "94",
  number           =  "3",
  pages		= "455--459",
  year		= "1985"
}

@article{Ve82,
  author		= "Veech, W.",
  title			= "Gauss measures for transformations on the space of interval exchange maps",
  journal		= "Ann. of Math. ",
  volume		= "115",
  number           =  "2",
  pages			= "201--242",
  year			= "1982"
}


@incollection {MR2931919,
    AUTHOR = {Veech, William A.},
     TITLE = {Invariant distributions for interval exchange transformations},
 BOOKTITLE = {Dynamical systems and group actions},
    SERIES = {Contemp. Math.},
    VOLUME = {567},
     PAGES = {191--219},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2012},
      ISBN = {978-0-8218-6922-2},
   MRCLASS = {37D40},
  MRNUMBER = {2931919},
MRREVIEWER = {Jon\ Chaika},
       DOI = {10.1090/conm/567/11254},
       URL = {https://doi.org/10.1090/conm/567/11254},
}

@article {athfor,
    AUTHOR = {Athreya, J. S. and Forni, G.},
     TITLE = {Deviation of ergodic averages for rational polygonal
              billiards},
   JOURNAL = {Duke Math. J.},
  FJOURNAL = {Duke Mathematical Journal},
    VOLUME = {144},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {285--319},
      ISSN = {0012-7094,1547-7398},
   MRCLASS = {37D50 (32G15 37A10 37F30)},
  MRNUMBER = {2437681},
MRREVIEWER = {Serge\ E.\ Troubetzkoy},
       DOI = {10.1215/00127094-2008-037},
       URL = {https://doi.org/10.1215/00127094-2008-037},
}

%% Journal article
@article{BS14,
  author		= "Bufetov, A.~I. and Solomyak, B.",
  title			= "On the modulus of continuity for spectral measures in substitution dynamics",
  journal		= "Adv. Math.",
  volume		= "260",
  pages			= "84--129",
  year			= "2014"
}

@article{BS18,
  author		= "Bufetov, A.~I. and Solomyak, B.",
  title			= "The {H}{\"o}lder property for the spectrum of translation flows in genus two",
  journal		= "Israel J. Math.",
  volume		= "223",
  pages			= "205--259",
  year			= "2018"
}


@article{BS20,
  author		= "Bufetov, A.~I. and Solomyak, B.",
  title			= "A spectral cocycle for substitution systems and translation flows",
  journal		= "J. Anal. Math.",
  volume		= "141",
  pages			= "165--205",
  year			= "2020"
}


@article {BS21,
    AUTHOR = { Bufetov, Alexander I. and Solomyak, B.},
     TITLE = {H\"older regularity for the spectrum of translation flows},
   JOURNAL = {J. Ecole polytechnique},
  FJOURNAL = {Journal de l’\'Ecole polytechnique--Math\'ematiques},
    VOLUME = {8},
      YEAR = {2021},
     PAGES = {279--310},
       DOI = {10.5802/jep.146.},
       URL = {https://jep.centre-mersenne.org/articles/10.5802/jep.146/},
}

@article {BS22,
    AUTHOR = { Bufetov, Alexander I. and Solomyak, B.},
     TITLE = {Corrigendum to ``H\"older regularity for the spectrum of translation flows''},
   JOURNAL = {J. Ecole polytechnique},
  FJOURNAL = {Journal de l’\'Ecole polytechnique--Math\'ematiques},
    VOLUME = {9},
      YEAR = {2022},
     PAGES = {1513--1514},
       DOI = {10.5802/jep.212.},
       URL = {https://jep.centre-mersenne.org/articles/10.5802/jep.212/},
}

@article {Fo22,
    AUTHOR = {Forni, G.},
     TITLE = {Twisted translation flows and effective weak mixing},
   JOURNAL = {J. Eur. Math. Soc.},
  FJOURNAL = {Journal of European Mathematical Society},
    VOLUME = {24},
    NUMBER = {12},
      YEAR = {2022},
     PAGES = {4225--4276},
       DOI = {10.4171/JEMS/1186},
}

@article {AFS23,
 AUTHOR = {Avila, A. and Forni, G. and Safaee, P.},
TITLE ={Quantitative weak mixing for interval exchange transformations}, 
  JOURNAL = {GAFA},
  FJOURNAL = {Journal
Geometric and Functional Analysis},
 YEAR ={2023},
 VOLUME = {33}, 
NUMBER = {1},
PAGES ={ 1--56},
ISBN ={1420-8970},
URL={
https://doi.org/10.1007/s00039-023-00625-y}, 

}

@article {Kat80,
 AUTHOR = {Katok, A.},
TITLE ={Interval exchange transformations and some special flows are not mixing}, 
  JOURNAL = {Israel J. Math.},
  FJOURNAL = {Israel Journal of Mathematics},
 YEAR ={1980},
 VOLUME = {35}, 
NUMBER = {4},
PAGES ={301--310},
ISBN ={1565-8511},
DOI ={10.1007/BF02760655},
URL={
https://doi.org/10.1007/BF02760655}, 

}

@inproceedings{MT02,
  author		= "Masur, H. and Tabachnikov, S.",
  title			= "Rational billiards and flat structures",
  editor		= "Hasselblatt, B. and Katok, A.",
  volume		= "1A",
  booktitle		= "Handbook of Dynamical Systems",
  pages		= "1015--1089",
   address		= "Amsterdam",
  publisher		= "Elsevier",
  year		= "2002"
}

@article{Ha44,
  author		= "Halmos, P. R.",
  title			= "In general a measure preserving transformation is mixing",
  journal		= "Ann. of Math.",
  volume		= "45",
  pages			= "786--792",
  year			= "1944"
}


@article{Ro48,
  author		= "Rokhlin, V.",
  title			= "A `general' measure-preserving transformation is not mixing (Russian)",
  journal		= "Dokl Akad Nauk SSSR (NS)",
  volume		= "60",
  pages			= "349--351",
  year			= "1948"
}

@article{FK36,
  author		= "Fox, R.~H. and Kershner, R.~B.",
  title			= "Concerning the transitive properties of geodesics on a rational polyhedron",
  journal		= "Duke Math. J.",
  volume		= "2",
  number           =  "1",
  pages			= "147-150",
  year			= "1936"
}

@article{RB81,
author = {Richens, P. J.  and Berry, M. V.},
title = {Pseudointegrable systems in classical and quantum mechanics},
journal = {Physica D: Nonlinear Phenomena},
volume = {2},
number = {3},
pages = {495-512},
year = {1981},
issn = {0167-2789},
doi = {https://doi.org/10.1016/0167-2789(81)90024-5},
url = {https://www.sciencedirect.com/science/article/pii/0167278981900245},
}

@article{KZ75,
  author		= "Katok, A.~B. and Zemlyakov, A.~M.",
  title			= "Topological transitivity of billiards in polygons",
  journal		= "Math. Notes of the Academy of Sciences of the USSR",
  volume		= "18",
  note                = "Errata {\bf 20} (1976), 1051",
  pages			= "760--764",
  year			= "1975"
}

@incollection{Kat_05, 
place={Cambridge}, 
series={London Mathematical Society Lecture Note Series}, 
title={Billiard table as a playground for a mathematician}, 
booktitle={Surveys in Modern Mathematics}, 
publisher={Cambridge University Press}, 
author={Katok, A. B.}, 
editor={Prasolov, Victor and Ilyashenko, YulijEditors}, 
year={2005}, 
pages={216–242}, 
collection={London Mathematical Society Lecture Note Series}} <div></div>


@article{BKM,
author = {Boldrighini, C. and Keane, M. and Marchetti, F.},
title = {Billiards in Polygons},
journal = {The Annals of Probability},
volume = {6},
number = {4},
pages = {532--540},
year = {1978},
url = {http://www.jstor.org/stable/2243120},
}

@article{Ra79,
author = {Rauzy, G.},
journal = {Acta Arithmetica},
keywords = {interval exchange transformation; minimality; unique ergodicity; induced transformations},
language = {fre},
number = {4},
pages = {315-328},
title = {\'Echanges d'intervalles et transformations induites},
url = {http://eudml.org/doc/205613},
volume = {34},
year = {1979},
}


@article{CE15,
author = {Chaika, J. and  Eskin, A.},
journal = {Journal of Modern Dynamics},
number = {1},
pages = {1--23},
title = {Every flat surface is Birkhoff and Oseledets generic in almost every direction},
url = {http://eudml.org/doc/205613},
volume = {9},
year = {2015},
doi = {10.3934/jmd.2015.9.1},
}

@inproceedings{Ko97,
 author		= "Kontsevich, M.",
 title			= "Lyapunov exponents and {H}odge theory",
 editor                =" ",
 volume		= "24",
 booktitle		= "The Mathematical Beauty of Physics (Saclay, 1996), Adv. Ser. Math. Phys.",
  pages		= "318--332",
  address		= "River Edge, NJ",
  publisher		= "World Sci. Publ.",
 year		= "1997"
}

@misc{KZ97, 
  author		= "Kontsevich, M. and Zorich, A.",
  title			= "Lyapunov exponents and {H}odge theory", 
  year			= "1997",
  note			= "Preprint at \url{https://arxiv.org/pdf/hep-th/9701164.pdf}"
}
  
@article{F02,
  author		= "Forni, G. ",
  title			= "Deviation of ergodic averages for area-preserving flows on surfaces of higher genus",
  journal		= "Ann. of Math.",
  volume		= "155",
  number           = "1",
  pages			= "1--103",
  year			= "2002"
}

%% Journal article
@article{F11,
  author		= "Forni, G. ",
  title			= "A geometric criterion for the nonuniform hyperbolicity of the {K}ontsevich--{Z}orich cocycle",
  journal		= "J. {M}od. {D}ynam.",
  volume		= "5",
  number           = "2",
  pages			= "355--395",
  year			= "2011"
}

@inproceedings{F06,
  author		= "Forni, G.",
  title			= "On the {L}yapunov exponents of the {K}ontsevich--{Z}orich cocycle",
  editor		= "Hasselblatt, B. and Katok, A.",
  volume		= "1B",
  booktitle		= "Handbook of Dynamical Systems",
  pages			= "549--580",
  address		= "Amsterdam",
  publisher		= "Elsevier",
  year			= "2006"
}

@article{AV07,
  author		= "Avila, A. and Viana, M.",
  title			= "Simplicity of {L}yapunov spectra: proof of the {Z}orich--{K}ontsevich conjecture",
  journal		= "Acta Math.",
  volume		= "198",
  number           = "1",
  pages			= "1--56",
  year			= "2007"
}

@article{Zo97, title={Deviation for interval exchange transformations}, volume={17}, DOI={10.1017/S0143385797086215}, number={6}, journal={Ergodic Theory and Dynamical Systems}, author={Zorich, A.}, year={1997}, pages={1477–1499}} <div></div>

@article{Vo97,
  author		= "Vorobets, Y.",
  title			= "Ergodicity of billiards in polygons",
  journal		= "Sb. Math.",
  volume		= "188",
  number           =  "3",
   note               = "(English translation of Mat. Sb. \textbf{188}, no. 3 (1997), 65--112)",
  pages		= "389--434",
  year		= "1997"
}

@ARTICLE{Fil16, 
  author = {Filip, Simion}, 
  title = {Semisimplicity and rigidity of the {K}ontsevich-{Z}orich cocycle}, 
  journal = {Invent. Math.}, 
  fjournal = {Inventiones Mathematicae}, 
  volume = {205}, 
  year = {2016}, 
  number = {3}, 
  pages = {617--670}, 
  issn = {0020-9910}, 
  mrclass = {32G20 (14D07 30F60 37D40)}, 
  mrnumber = {3539923}, 
  mrreviewer = {Christian Schnell}, 
  doi = {10.1007/s00222-015-0643-3}, 
  url = {https://doi.org/10.1007/s00222-015-0643-3}, 
  zblnumber = {1368.14013}, 
  }
@incollection{FCet, 
place={Cetraro}, 
series={Lecture Notes in Mathematics (LNM)-CIME Foundation Subseries}, 
title={Effective Unique Ergodicity and Weak Mixing of Translation Flows}, 
booktitle={Modern Aspects of Dynamical Systems}, 
publisher={Springer}, 
author={Forni, G.}, 
editor={C. Bonanno, C. Sorrentino, C. Ulcigrai }, 
year={2024},
pages={161--221}, 
volume={2347}
} 


@book{DT02, place={Cambridge}, series={Cambridge Monographs on Applied and Computational Mathematics}, title={Schwarz-Christoffel Mapping}, publisher={Cambridge University Press}, author={Driscoll, Tobin A. and Trefethen, Lloyd N.}, year={2002}, collection={Cambridge Monographs on Applied and Computational Mathematics}} <div></div>



@ARTICLE{CH, 
  author = {Chaika, J. and Hubert, P.}, 
  title = {Circle averages and disjointness in typical translation surfaces on every Teichm\"uller disc}, 
  journal = {Bull. London Math. Soc. }, 
  fjournal = {Bulletin of the London Mathematical Society}, 
  volume = {49}, 
  year = {2017}, 
  number = {5}, 
  pages = {755--769}, 
  issn = {}, 
  mrclass = { }, 
  mrnumber = {}, 
  mrreviewer = {}, 
  doi = {https://doi.org/10.1112/blms.12065}, 
  url = {https://londmathsoc.onlinelibrary.wiley.com/doi/abs/10.1112/blms.12065}, 
  zblnumber = {}, 
  }
